Fock State Sampling Method -- Characteristic temperature of maximal fluctuations for interacting bosons in box potentials

We study the statistical properties of a gas of interacting bosons trapped in a box potential in two and three dimensions. Our primary focus is the characteristic temperature $\tchar$, i.e. the temperature at which the fluctuations of the number of condensed atoms (or, in 2D, the number of motionless atoms) is maximal. Using the Fock State Sampling method, we show that $\tchar$ increases due to interaction. In 3D, this temperature converges to the critical temperature in the thermodynamic limit. In 2D we show the general applicability of the method by obtaining a generalized dependence of the characteristic temperature on the interaction strength. Finally, we discuss the experimental conditions necessary for the verification of our theoretical predictions.

==> answer.tex <==

We thank the referee for their valuable comments.

Following the first suggestion, we decided to change the title  to "Fock State Sampling Method -- Characteristic temperature of maximal fluctuations for interacting bosons in box potentials"

Furthermore, we have also introduced remarks concerning the role of superposition, adding the text 
"It has two consequences. First, it neglects the phenomenon of quantum depletion. Thus, the method is expected to yield correct results only for weak interactions. Second, it is not applicable to weakly interacting bosons confined by the harmonic trap, since, in this case, the condensate wavefunction is a superposition of many oscillator states."

We also improved Fig. 3 focusing on the results for the interacting systems.
